Scaling Nakamoto Consensus to Thousands of Transactions per Second

This paper presents Conflux, a fast, scalable and decentralized blockchain system that optimistically process concurrent blocks without discarding any as forks. The Conflux consensus protocol represents relationships between blocks as a direct acyclic graph and achieves consensus on a total order of the blocks. Conflux then, from the block order, deterministically derives a transaction total order as the blockchain ledger. We evaluated Conflux on Amazon EC2 clusters with up to 20k full nodes. Conflux achieves a transaction throughput of 5.76GB/h while confirming transactions in 4.5-7.4 minutes. The throughput is equivalent to 6400 transactions per second for typical Bitcoin transactions. Our results also indicate that when running Conflux, the consensus protocol is no longer the throughput bottleneck. The bottleneck is instead at the processing capability of individual nodes.

==> App_Proof.tex <==
\newcommand{\setlmaref}[1]{\setcounterref{relemma}{#1}\addtocounter{relemma}{-1}}

\newtheorem{relemma}{Lemma}
\newtheorem{retheorem}[relemma]{Theorem}

\section{Proof of correctness}
\label{app:proof}

\subsection{Proof of lemma \ref{lem:confirm}}
\setlmaref{lem:confirm}
\begin{relemma}
	Suppose $b$ is a block on the pivot chain of all honest nodes during the
	time $[t-d, t]$ and $P(b)$, the parent of $b$, is generated at time zero. The
	chance of $b$ being kicked out of the pivot chain by one of its sibling block
	$a$ is:
	\begin{displaymath}
	\sum_{k=0}^{n-m}\zeta_k \cdot q^{n-m-k+1} + \sum_{k=n-m+1}^{\infty} \zeta_k
	\end{displaymath}
	where $n$ is the number of blocks in the subtree of $b$ before time $t-d$, $m$ is the number of blocks in the subtree of $a$ 
	generated by honest nodes, and $\zeta_k = e^{-q\lh t}\frac{(q\lh t)^k}{k!}$.
\end{relemma}

\begin{proof}
    We use $G_t^v$ to denote the local state of participant $v$ at global time
    $t$. $G^\infty_t$ is the union set of the local state of all the
    participants (including attacker). $G^\mathrm{honest}_t$ is the union set
    of all the honest participants' local state. 
	
    While all honest participants are acknowledging $b$ as pivot block, the
    expected waiting time for the next strengthening subtree of $b$ is $1/\lh$.

    Now consider an honest participant in the worst network case: every blocks
    in the subtree of $b$ have the maximum delay $d$, but the blocks in other
    subtrees have no delay. If $a$ haven't kicked out of $b$ in this
    participant, it won't revert $b$ at any honest node. 

    In the node with the worst network case, the gap between pivot block $b$
    and its sibling $a$ are
    $X_0=|\mathrm{Desc}(G^\infty_{t-d},b)|-|\mathrm{Desc}(G^\mathrm{honest}_{t},a)|.$
    According to theorem 10 in \cite{GHOST}, attacker can extend $a$ to be
    weighter than $b$ with probability less than
    $\left(\frac{q\lh}{\lh}\right)^{X_0+1}$.

    Let $m=\mathrm{Desc}(G^\mathrm{honest}_{t},a)$,
    $n=\mathrm{Desc}(G^\infty_{t-d},b)$, $k$ be number of blocks generated
    later than time zero. Then we can claim
    $|\mathrm{Desc}(G^\mathrm{\infty}_{t},a)|\le k+m$, $X_0\ge n-m-k$. The
    probability of generate $k$ attacker blocks in time $t$ is $\zeta_k =
    e^{-q\lh t}\frac{(q\lh t)^k}{k!}$, the chance of $b$ being kicked out of
    the pivot chain by its sibling $a$ is less than $$ \sum_{k=0}^{\infty}
    \zeta_k \cdot \min\left\{q^{n-m-k+1},1\right\}.$$ \end{proof}

\subsection{Proof of theorem \ref{the:confirm}}
\setlmaref{the:confirm}
\begin{retheorem}
	Suppose $b$ is a block on the pivot chains of all honest nodes during the time $[t-d, t]$.
	The chance of $b$ falls off the pivot chain is less than:
	\begin{displaymath}
	\max_{\substack{a\in \mathrm{Chain}(G,b)\\ a'\in \mathrm{Sibling}(a)}} \mathrm{Pr}[\text{$a$ is kicked out of the pivot chain by $a'$}]
	\end{displaymath}
\end{retheorem}
\begin{proof}
    For any time $t'>t$, let $m(t')$ be the blocks generated by attacker in
    $[t, t']$, $n(t')$ be the blocks generated by honest participants in $[t,
    t'-d]$. If the attacker reverts pivot block $\bar{a}\in \mathrm{Past}(G,b)$
    by $\bar{a}'\in \mathrm{Sibling}(\bar{a})$ at time $t'$. We can claim
    \begin{align*}
		 &m(t')-n(t') \\
		> & |\mathrm{Desc}(G^\infty_{t},\bar{a})|-|\mathrm{Desc}(G^\mathrm{\infty}_{t},\bar{a}')| \\
		\ge & \min_{\substack{a\in \mathrm{Chain}(G,b)\\ a'\in \mathrm{Sibling}(a)}} |\mathrm{Desc}(G^\infty_{t},a)|-|\mathrm{Desc}(G^\mathrm{\infty}_{t},a')|
	\end{align*}
	
    We use $k$ denote $$\min_{\substack{a\in \mathrm{Chain}(G,b)\\ a'\in
            \mathrm{Sibling}(a)}}|\mathrm{Desc}(G^\infty_{t},a)|-|\mathrm{Desc}(G^\mathrm{\infty}_{t},a')|.$$

     So $m(t')-n(t')>k$ is the necessary condition for a successful attack
     under any strategies.

     If the attacker chooses $\tilde{a},\tilde{a}'$ which minimize $k$ and
     mines blocks under $\tilde{a}'$, $m(t')-n(t')>k$ is also the sufficient
     condition. Since $m(t')$ and $n(t')$ are independent with strategies,
     mining blocks under $\tilde{a}'$ is the dominant strategy for attacker. So
     the successful probability is dominate by the probability of reverting the
     most competitive $\tilde{a}'$.
\end{proof}

\noindent \textbf{Remark:} The probability space of lemma \ref{lem:confirm} and
theorem \ref{the:confirm} are different. In  lemma \ref{lem:confirm}, we
estimate the probability given subtree size $m$ and $n$. In theorem
\ref{the:confirm}, we estimate the probability given all the blocks generated
before time $t$.


==> figs/raw1.tex <==
\begin{sidewaystable*}
\scriptsize
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
Consensus & Block Size & Gen. Interval & D & Latency (min) & L (25\%) & L (medium) & L (75\%) & L (Max) & Chain Ratio & Achieved TPT (MB/s) & Header Overhead & Real TPT (MB/s) \\
\hline
Bitcoin & 1MB & 10min &  &  &  &  &  &  &  &  &  &  XXX \\
\hline
Bitcoin & 8MB & 20s & 165.38 & 1883.86 & 2097.25 & 2144.02 & 2232.37 & 2399.79 & 0.481 & 0.192 &  &  XXX \\
\hline
Bitcoin & 4MB & 20s & 108.33 & 621.40 & 801.54 & 866.72 & 923.44 & 1104.36 &  0.633 & 0.127 &  &  XXX \\
\hline
Bitcoin & 2MB & 20s  & 80.35 & 411.64 & 531.66 & 603.63 & 669.64 & 873.98 & 0.731 &  0.0731&  &  XXX \\
\hline
Bitcoin & 1MB & 20s & 44.90 & 288.18 & 392.91 & 435.15 & 470.73 & 570.33 & 0.794 & 0.0436 &  &  XXX \\
\hline
Bitcoin & 4MB & 10s & 116.43 & 1394.92 & 1474.19 & 1507.77 & 1546.37 & 1612.74 & 0.433 & 0.189 & 251 Byte &  XXX \\
\hline
Bitcoin & 4MB & 20s & 108.33 & 621.40 & 801.54 & 866.72 & 923.44 & 1104.36 &  0.633 & 0.127 &  &  XXX \\
\hline
Bitcoin & 4MB & 40s  & 70.09 & 677.94 & 785.76 & 986.26 & 1138.82 & 1414.49 & 0.772 & 0.0824 & 251 Byte &  XXX \\
\hline
Bitcoin & 4MB & 80s  & 55.97 & 1540.23 & 1728.83 & 2066.66 & 2398.00 & 2804.29 & 0.833 & 0.0373 &  &  XXX \\
\hline
GHOST & 8MB & 20s & 142.07 &  535.101581 &813.09 &936.34 &1071.92 &1387.44  &  0.436& 0.190 &  &  XXX \\
\hline
GHOST & 4MB & 20s & 87.19 & 205.99 & 305.27 & 479.25 & 636.81 & 932.80 & 0.625 &  0.129& &  XXX \\
\hline
GHOST & 2MB & 20s  & 22.25 & 117.03 & 219.77 & 310.70 & 404.95 & 576.87 & 0.806 & 0.768 &  &  XXX \\
\hline
GHOST & 1MB & 20s  & 30.17 & 35.60 & 166.06 & 244.58 & 305.64 & 585.98 & 0.856 & 0.0440 &  &  XXX \\
\hline
GHOST & 4MB & 10s & 132.79 & 283.96 & 409.99 & 548.00 & 665.96 & 833.70 & 0.436 & 0.186 &  &  XXX \\
\hline
GHOST & 4MB & 20s & 87.19 & 205.99 & 305.27 & 479.25 & 636.81 & 932.80 & 0.625 &   0.129& &  XXX \\
\hline
GHOST & 4MB & 40s  & 98.09 & 310.58 & 529.94 & 748.59 & 941.46 & 1416.60 & 0.778 & 0.0701 &  &  XXX \\
\hline
GHOST & 4MB & 80s  & 19.857304 & 348.65 & 853.37 & 1106.18 & 1379.90 & 2061.39 & 0.9 & 0.039 &  &  XXX \\
\hline
{\name} & 8MB & 20s &  148.46 &711.49&1017.98&1089.75&1185.69&1509.82& 0.442 & 0.400  &  &  XXX \\
\hline
{\name} & 4MB & 20s & 71.34 &  168.28 &399.04 &528.90 &657.52&931.49  &0.614 & 0.211 &  &  XXX \\
\hline
{\name} & 2MB & 20s  & 19.23 &  83.22 &220.25 &322.25 &401.94 &722.82  & 0.764 & 0.420 &  &  XXX \\
\hline
{\name} & 1MB & 20s  & 24.28 &  67.850434 &145.07 &237.39 &322.40 &595.63 & 0.828 & 0.0541 &  &  XXX \\
\hline
{\name} & 4MB & 10s &  92.13 & 266.44& 482.00 &590.63 &691.02 &909.62 & 0.444& 0.400 &  &  XXX \\
\hline
{\name} & 4MB & 20s &  71.31 &  168.28 &399.04 &528.90 &657.52 &931.49 & 0.614 & 0.211 &  &XXX \\
\hline
{\name} & 4MB & 40s  & 69.03 &  211.18& 401.75 &476.96& 570.43 &814.23& 0.806 & 0.111 &  &  XXX \\
\hline
{\name} & 4MB & 80s  & 69.73 &  272.264 &496.83 &809.69 &1042.14 &1754.00 & 0.822& 0.054 &  &  XXX \\
\hline
{\name} & 4MB & 5s  & 138.03 &  1223.09 &1404.51 &1456.53 &1503.37 &2031.15 & 0.257& 0.96 &  &  XXX \\
\hline
\end{tabular}
\caption{Fix 10k users. Assume attacker controls no more than 20\% when calculating latency with 0.01\% tolerence.}
\end{sidewaystable*}



==> figs/raw2.tex <==
\begin{sidewaystable*}
\scriptsize
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
User\# & Block Size & Gen. Interval & D & Latency (min) & L (25\%) & L (medium) & L (75\%) & L (Max) & Chain Ratio & Achieved TPT (MB/s) & Header Overhead & Real TPT (MB/s) \\
\hline
2.5k & 4MB & 20s & 69.90 &175.40&336.72&459.20&562.59&1000.76  &  0.625 & 0.211 & & XXX \\
\hline
5k & 4MB & 20s & 69.31&166.05&322.14&438.61&538.48&919.61&0.669 & 0.398 &  &  XXX \\
\hline
10k & 4MB & 20s &  71.31 &  168.28 &399.04 &528.90 &657.52 &931.49 & 0.614 & 0.211 &  &XXX \\
\hline
20k & 4MB & 20s  & 74.61&179.85&353.74&432.81&508.58&803.16&0.636 & 0.214 &  &  XXX \\
\hline
\end{tabular}
\caption{Change the number of users from 2.5k to 10k. Fix 4M and 20s.}
\end{sidewaystable*}



==> figs/total-order.tex <==
\begin{algorithm}[t]
\small
\SetNlSty{}{}{}
\DontPrintSemicolon
\SetKw{To}{ to }
\SetKw{In}{ in }
\SetKw{And}{ and }
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{The local state $G = \langle B, g, P, E \rangle$}
\Output{An ordered list $L$ of a subset of blocks in $G$ }
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line

$a \longleftarrow \mathrm{Pivot}(G)$\;
\Return $\mathrm{DaggerOrder}(G,a)$\;
\caption{The {\name} Total Order $\TO(G)$}
\label{fig:total-order}
\end{algorithm}


==> figs/weight.tex <==
\begin{algorithm}[t]
\small
\SetNlSty{}{}{}
\DontPrintSemicolon
\SetKw{To}{ to }
\SetKw{In}{ in }
\SetKw{And}{ and }
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\SetKw{Define}{define}
\Input{The local state $G = \langle B, g, P, E \rangle$, a block $b \in B$, and the parallel parameter $k$}
\Output{The $k$-parallel weight of the subtree of $b$}
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line

$U \longleftarrow B \cap \mathrm{Subtree}(G, b)$\;
\Define $\mathrm{ParaD}(G, U, b') = |\{b'' \mid b'' \in U \cap \mathrm{Para}(G, b')\}|$\;
$k' \longleftarrow \max_{b' \in U} {\mathrm{ParaD}(G, U, b')}$\;
\While {$k' > k$} {
    $C \longleftarrow \{ b' \mid \mathrm{ParaD}(G, U, b') = k'\}$\;
    $t \longleftarrow \mathrm{arg\,min}_{b' \in C} {\mathrm{Hash}(b')}$\;
    $U \longleftarrow U - \{t\}$\;
    $k' \longleftarrow \max_{b' \in U} {\mathrm{ParaD}(G, U, b')}$
}
\Return $|U|$\;
\caption{The definition of $\mathrm{Weight}(G, k, b)$}
\label{fig:weight}
\end{algorithm}


==> honest-decendent.tex <==
\begin{algorithm}[t]
	\small
	\SetNlSty{}{}{}
	\DontPrintSemicolon
	\SetKw{To}{ to }
	\SetKw{In}{ in }
	\SetKw{And}{ and }
	\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
	\Input{The local state $G = \langle B, g, P, E \rangle$, two aim block $b_1,b_2$, the maximum forward delay $D$}
	\Output{Estimate maximum number of honest decedents}
	\let\oldnl\nl% Store \nl in \oldnl
	\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
	
	We use $\mathrm{Desc}(G,a,T)$ denote $\{b\;|\;b\in\mathrm{DescP}(G,a,T) \text{ and } b.\mathsf{time} \le T\}$.
	
	$T' \leftarrow \max\{T\;|\;|\mathrm{DescP}(G,b_1,T-2D)|>|\mathrm{DescP}(G,b_2,T)|\}$
	
	\Return $|\mathrm{DescP}(G,b_2,T')|$
	\caption{The Definition of $\mathrm{DescBound}(G,b_1,b_2,D)$}
	\label{fig:prefix-choice}
\end{algorithm}


==> prefix-choice.tex <==
\begin{algorithm}[t]
\small
\SetNlSty{}{}{}
\DontPrintSemicolon
\SetKw{To}{ to }
\SetKw{In}{ in }
\SetKw{And}{ and }
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{The local state $G=G^v$, the risk tolerance $r$ of recipient, the honest node generation rate $\lh$, the attacker ratio $q$, the local time stamp $T$, the maximum forward delay $D$.}
\Output{A list of blocks $L = b_1 \circ b_2 \circ \ldots \circ b_n$, where $b_1 = g$}
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line

$a\leftarrow\mathrm{Pivot}(G_T)$\;

\Repeat{$a= g$} {
	\If {$T-P(a).\tm\le 3D$} {
		$a\leftarrow \mathrm{Before}(G_T,a)$\;
		\textbf{Continue}\;
	}
	$n\leftarrow |\mathrm{Desc}(G_{T-2D},a)|$\;
	$t \leftarrow T- P(a).\mathsf{time}-D$\;
	
	$\lambda \leftarrow q\lh t$\;
	$s\leftarrow 1$\;
	\For{Each $b\in\mathrm{Child}(G,P(a))$ which $b\neq a$}{
		\If{$ |\mathrm{Desc}(G_T,b)|<|\mathrm{Desc}(G_{T-3D},a)|$}{
			$s\leftarrow 0$\;
			\textbf{break}\;
		} 
		$m\leftarrow|\mathrm{DescHonest}(G_T,b)|$\;
		$s' \leftarrow \sum_{k=0}^{n-m} e^{- \lambda}\cdot\frac{\lambda^k}{k!}\cdot (1-q^{n-m-k+1})$\;
		$s\leftarrow \min\{s,s'\}$\;
	}
	
	$a.\mathsf{risk}\leftarrow 1-s$\;
	$a\leftarrow\mathrm{Before}(G_T,a)$\;
}
	Let $a'$ be the earliest block such that $a'.\mathsf{risk}\ge r$

\Return The prefix of $\TO(G)$ from $g$ to $\mathrm{Past}(G_T,a')$.
\caption{The Definition of $\TOP(G,r,\lh,q,T,D)$}
\label{fig:prefix-choice}
\end{algorithm}

